An O(a) modified lattice set-up of the Schr\"odinger functional in SU(3) gauge theory

The set-up of the QCD Schr\"odinger functional (SF) on the lattice with staggered quarks requires an even number of points $L/a$ in the spatial directions, while the Euclidean time extent of the lattice, $T/a$, must be odd. Identifying a unique renormalisation scale, $L=T$, is then only possible up to O($a$) lattice artefacts. In this article we study such lattices in the pure SU(3) gauge theory, where we can also compare to the standard set-up. We consider the SF coupling as obtained from the variation of an SU(3) Abelian and spatially constant background field. The O($a$) lattice artefacts can be cancelled by the existing O($a$) boundary counterterm. However, its coefficient, $\ct$, differs at the tree-level from its standard value, so that one first needs to re-determine the induced background gauge field. The perturbative one-loop correction to the coupling allows to determine $\ct$ to one-loop order. A few numerical simulations serve to demonstrate that residual cutoff effects in the step scaling function are small in both cases, $T=L\pm a$ and comparable to the standard case with $T=L$.

==> fig_tab/table_m1_data_nu1.tex <==
\begin{tabular}{|c|l|l|l|}
 \hline 
 \hline
$L/a $ & $ s=1 $& $s=0$ & $ s = 1$ \\ \cline{1 - 4} 
 $4$ & $0.675227287641726$ & $0.612284383798761$ & $0.603268035987959$  \\ 
$6$ &  $0.713688436927250$ & $0.667377115635360$ & $0.658661671430230$  \\ 
$8$ &  $0.746023908925775$ & $0.710038355834626$ & $0.703335892433600$  \\ 
$10$ & $0.772934184571797$ & $0.743677169992082$ & $0.738298337870965$  \\ 
$12$ & $0.795691819448238$ & $0.771092038835863$ & $0.766605582990425$  \\ 
$14$ & $0.815337982963828$ & $0.794135893575063$ & $0.790288798373617$  \\ 
$16$ & $0.832598987596293$ & $0.813979394683868$ & $0.810612469726827$  \\ 
$18$ & $0.847982016011203$ & $0.831389217162389$ & $0.828396027720952$  \\ 
$20$ & $0.861851017995113$ & $0.846890045075210$ & $0.844195970633759$  \\ 
$22$ & $0.874474765273853$ & $0.860855207150777$ & $0.858405928015078$  \\ 
$24$ & $0.886056918523759$ & $0.873559186401280$ & $0.871313938923100$  \\ 
$26$ & $0.896755288193035$ & $0.885209412694253$ & $0.883136828015203$  \\ 
$28$ & $0.906694540326568$ & $0.895966322039620$ & $0.894041746563870$  \\ 
$30$ & $0.915974819966177$ & $0.905956481638081$ & $0.904160188678965$  \\ 
$32$ & $0.924677757522087$ & $0.915281454158502$ & $0.913597413603667$  \\ 
$34$ & $0.932870750815903$ & $0.924023952167856$ & $0.922438961298534$  \\ 
$36$ & $0.940610081359162$ & $0.932252215394830$ & $0.930755271025231$  \\ 
$38$ & $0.947943224677001$ & $0.940023191170245$ & $0.938605026881105$  \\ 
$40$ & $0.954910592045031$ & $0.947384888932024$ & $0.946037627993324$  \\ 
$42$ & $0.961546862352023$ & $0.954378153197309$ & $0.953095043765602$  \\ 
$44$ & $0.967882015642729$ & $0.961038018825855$ & $0.959813229603927$  \\ 
$46$ & $0.973942143221024$ & $0.967394759995257$ & $0.966223220155886$  \\ 
$48$ & $0.979750091974123$ & $0.973474714855775$ & $0.972351987246859$  \\ 
$50$ & $0.985325979547273$ & $0.979300937314023$ & $0.978223117315728$  \\ 
$52$ & $0.990687611515399$ & $0.984893720945901$ & $0.983857354460644$  \\ 
$54$ & $0.995850822868038$ & $0.990271022189279$ & $0.989273038551004$  \\ 
$56$ & $1.000829757948720$ & $0.995448805011554$ & $0.994486462997682$  \\ 
$58$ & $1.005637102211141$ & $1.000441324866937$ & $0.999512166571981$  \\ 
$60$ & $1.010284275908234$ & $1.005261364520710$ & $1.004363177878588$  \\ 
$62$ & $1.014781598138714$ & $1.009920429831240$ & $1.009051216677276$  \\ 
$64$ & $1.019138420885904$ & $1.014428911943546$ & $1.013586861389271$  \\ 
\hline 
 \hline 
\end{tabular}


         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         
         


